SSL-WM: A Black-Box Watermarking Approach for Encoders Pre-trained by Self-supervised Learning

Recent years have witnessed tremendous success in Self-Supervised Learning (SSL), which has been widely utilized to facilitate various downstream tasks in Computer Vision (CV) and Natural Language Processing (NLP) domains. However, attackers may steal such SSL models and commercialize them for profit, making it crucial to verify the ownership of the SSL models. Most existing ownership protection solutions (e.g., backdoor-based watermarks) are designed for supervised learning models and cannot be used directly since they require that the models' downstream tasks and target labels be known and available during watermark embedding, which is not always possible in the domain of SSL. To address such a problem, especially when downstream tasks are diverse and unknown during watermark embedding, we propose a novel black-box watermarking solution, named SSL-WM, for verifying the ownership of SSL models. SSL-WM maps watermarked inputs of the protected encoders into an invariant representation space, which causes any downstream classifier to produce expected behavior, thus allowing the detection of embedded watermarks. We evaluate SSL-WM on numerous tasks, such as CV and NLP, using different SSL models both contrastive-based and generative-based. Experimental results demonstrate that SSL-WM can effectively verify the ownership of stolen SSL models in various downstream tasks. Furthermore, SSL-WM is robust against model fine-tuning, pruning, and input preprocessing attacks. Lastly, SSL-WM can also evade detection from evaluated watermark detection approaches, demonstrating its promising application in protecting the ownership of SSL models.

==> overview.tex <==
\section{Motivation}
\label{sec:Motivation}


\begin{figure}[t]
\centering
\epsfig{figure=fig/motivation.png, width=0.5\textwidth} 
\caption{\textbf{Motivation Example}}
\label{fig:motivation}
\end{figure}






\subsection{Threat Example}
\shengzhi{Motivation examples means you tell a story: a) A model owner releases their model (complicated and accurate) on github, b) adversary identifies its value and clones it, c. To avoid legal issues, adversary fine-tunes (XXX approaches) the model and adds his own watermark, d) Adversary commercializes it (make it black box as well) and gets revenue. Then you want to use the story to emphasize the need of our approach: a) black box model from adversary, so we need to probe. But since the model is complicated and adversary has done pruning, the results of probing may not be convincing. Therefore, white box verification is needed.}

As the advance of AI techniques, neural networks are involving in various complicated tasks, e.g., autonomous driving, speech recognition, remote diagnosis, etc. Such tasks usually rely on DNN models trained on a large amount of data using intensive GPU resources.
For instance, AlexNet paper[] it’s stated that “our network takes between five and six days to train on two GTX 580 3GB GPUs”. \shengzhi{Give an example of a real world complicated model trained using XXX data and XXX GPU for XXX days.} Hence, the IP of DNN models has become a vital topic in the AI community. 

Consider an example as shown in Figure\ref{fig:motivation}, Alice makes great efforts to design a complicated and accurate neural network $DNN_{Alice}$ that performs well on the main task, and embed a backdoor[] watermark to $DNN_{Alice}$. Then he publishes $DNN_{Alice}$ to models sharing platform, such as GitHub and Google Cloud AI platform []. After that, an attacker Bob thinks that $DNN_{Alice}$ is very valuable, and then stealing it. To avoid legal issues, Bob fine-tunes, prunes the model and adds his own backdoor[] watermark, generating $DNN_{Bob}$. Next, Adversary commercializes it in black box and gets revenue.  

In view of this situation, Alice needs to claim ownership of the stolen model $DNN_{Bob}$. Alice first performs black box verification on $DNN_{Bob}$, but at this time, Bob can also have some key samples constructed by AEs or from his new constructed backdoor for fraudulent claims of ownership. Moreover since the model is complicated and adversary has done pruning, the results of probing by backdoor may not be convincing. 

%\begin{figure}[t]
%\centering
%\epsfig{figure=fig/table_attacker.png, width=0.5\textwidth} 
%\caption{\textbf{Capability of Attacker}}
%\label{fig:table_attacker}
%\end{figure}

\begin{table}
\centering
\footnotesize
\caption{Capability of Watermark}
\label{tab:Capability of Attacker}
\begin{tabular}{m{2.5cm}
<{\centering}|m{1.5cm}
<{\centering}|m{1.5cm}
<{\centering}|m{1.4cm}
<{\centering}}
\hline
\textbf{ }& \textbf{Elementary level}& \textbf{Intermediate level}& \textbf{Advanced level}\\
\hline \hline
\textbf{Fraudulent claims of ownership} & \text{\Checkmark}& \text{\Checkmark}& \text{\Checkmark}\\ \hline
\textbf{Access to White Box}& \text{-} &\text{\Checkmark}& \text{\Checkmark} \\ \hline
\textbf{Pruning and Fine-tuning}& \text{-} &\text{-}& \text{\Checkmark} \\ \hline
\textbf{Watermark Rewrite}& \text{-} &\text{-}& \text{\Checkmark} \\ \hline
\end{tabular}
\end{table}

\shengzhi{The Table needs revision. It should show how existing works and ours perform on those metrics listed in the first column.}

Moreover, we classify several levels of attackers according to the capability our attacker can have as show in Figure \ref{fig:table_attacker}.
These attackers cause great challenges to current backdoor watermarking methods. Therefore, some watermark that can play an arbitration role in ownership verification is needed, we propose $HufuNet$ which can give an arbitration result of ownership in white box. Only in this way, can Alice verify the ownership of $DNN_{Bob}$ without any controversy.


\begin{comment}
A well-trained DNN is a valuable intellectual property (IP) for its owners, officials hope to use legal measures to protect the intellectual property of model owners. And the role of the watermark is primarily to protect the IP from being infringed.

The potential security risks of the IP of DNN are watermark removing and fraudulent claims of ownership. In terms of watermark removing, previous work \textcolor{red}{[leveage] [fine-prune] [evasion]} showed that attacker $\mathbb{A}$ can increase learning rates to fine-tuning or pruning to effectively remove the black box watermark. In terms of fraudulent claims of ownership, attacker $\mathbb{A}$ can generate some AEs [X] to fraudulent claim of ownership. Both of these risks are huge challenges to black box watermark. To address the above problems, we propose a new watermark ownership framework that provides the first black box verification, and then white box ownership verification with a high robustness protection mechanism.

For the $DNN_{valid}$ of disputed ownership, we first perform a robust black box watermark verification. If the verification result is under a high degree of confidence, we will prove the ownership of $DNN_{valid}$. But in the following two cases, the black box watermarking is not enough to verify ownership, and we will utilize the more robust and trustworthy white box watermarking method. 
(1)The black box method does not prove our ownership with a high degree of confidence, but we found out it is our model through a few minor details, and then we take legal means to get the white box model of $DNN_{valid}$ for further verification. (2)Fraudulent claims of ownership. Although we can verify ownership in the black box, attackers can also generate some adversarial samples and verify them in black box. 
Similarly, we take legal means to get the white box model of $DNN_{valid}$ and performs white box verification.
\end{comment}

\begin{comment}

\subsection{Threat Model}

\shengzhi{Usually threat model is to assume the maximum capability your adversary can have. Then your approch is to deal with the worse case based on your threat model.}

The main methods of attack to eliminate the DNN watermark are pruning, fine-tuning, and watermark rewriting. Also fraudulent clams ownership attack leads to disputes over ownership. As far as these attack methods proposed, We classify several levels of attackers $\mathbb{A}$ according to the maximum capability our attacker can have as follows:

Elementary level: $\mathbb{A}$ cannot get our white box model, nor has ability of pruning, fine-tuning, watermark rewrite to our model. But he claim the ownership of our DNN rascally without any evidience.

Intermediate level:$\mathbb{A}$ does not have access to our white box model. However, they generate some AEs through queries, which in turn build trigger sets to claim ownership of the black box DNN.

Advanced level: $\mathbb{A}$ can obtain the white box model, then without pruning, fine-tuning and rewriting watermark to model. $\mathbb{A}$ didn't embed the watermark, but claimed that part of the neural network was his watermark.

Ultimate level: $\mathbb{A}$ can get access to the white box model and perform operations such as pruning and fine-tuning, further adding a similar white box secret key to claim ownership.

\end{comment}



\subsection{Design Requirements}
\shengzhi{Based on the threat model, here you can elaborate the design requirements, e.g., effectiveness, fidelity, robustness, integrity, security, etc.}

As mentioned above, we assume that attackers have a certain amount of destructive power and therefore some technical challenges need to be addressed for achieve accurate and efficient verification of watermark ownership. We conducted an in-depth analysis of the capabilities of the four levels of attackers in order to propose an excellent watermark approach.
\begin{comment}
Elementary level: Since the attacker $\mathbb{A}$ cannot get our white box model and cannot build trigger sets to verify ownership in black box, we need to design a watermark with good quality of effectiveness and integrity and security in black box verification. 

\end{comment}

Elementary level: The attacker $\mathbb{A}$ can generate some AEs to generate his trigger sample to claim ownership of our DNN, even without access to our DNN. It is a drawback to backdoor watermark to defend the attack fraudulently claim ownership. So we need to design a new watermark total different from backdoor watermark to avoid the drawback of backdoor. The new watermark shall meet the requirement as: it only can  verify the ownership of DNN which it embedded; it is difficult to fake a substitute watermark to claim ownership.

Intermediate level: Owning $\mathbb{A}$ can obtain the white box DNN and claimed that a originally part of the DNN was his watermark. In this case, we must sure our watermark with quality that watermark is undetected by attacker and it is difficult to fake a substitute watermark only by some original part of DNN and attack's local secret.


Advanced level: Due to $\mathbb{A}$ gaining the white box model, and attacking our watermark by pruning, fine-tuning, and watermark rewriting. Therefore, we need to make sure the white box watermark is of good robust to these attacks and undetected by adversary.

Moreover, a well watermark should have guaranteed a good quality that after embedding watermark, the protected DNN can not have a significant decrease in performance.

\vspace{5pt}

==> sections/Implementation.tex <==
\section{Implementation.}
\label{sec:implementation}



\todo{VGGFace????}

==> sections/RelatedWork.tex <==
\section{Related Work}

\subsection{Backdoor Attacks in DNNs}
\label{subsec:backdoor-attack}
Gu et al.~\cite{gu2017badnets} first proposed the backdoor attack (i.e., Badnets) into DNNs, which injects backdoor by controlling the training process through polluting the training dataset with some poison data stamped with triggers (e.g., a sticker in the lower right corner of images) and relabelled to the target label, and the backdoored DNNs will misclassify the backdoor samples stamped with the trigger as the target label. However, Badnets needs to access the training dataset to backdoor DNNs, which doesn't apply to the data-free scenarios. Chen et al.~\cite{Targeted backdoor attacks on deep learning systems using data poisoning} proposed a blended strategy to generate the backdoor samples by blending the triggers (e.g., glasses) with the benign samples (e.g., faces) and use the poison dataset to train backdoor DNNs. However, this attack needs access to the training dataset and doesn't apply to the data-free cases. These poisoned training samples are all labeled to the target class, which could be detected as inconsistent by humans by examining the image-label relationship of training samples. To address it, poison frogs~\cite{poison frogs} first proposed the clean label attack, which leverages adversarial perturbations to modify some benign images from the target class via feature collisions with clean base samples and then conducted the attack using clean clean examples. Then, Zhu et al.~\cite{Transferable Clean-Label Poisoning Attacks on Deep Neural Nets} proposed a transferable clean label poisoning attack that succeeds without access to the DNNs' architecture, outputs, or training data. Afterward, Zhao et al.~\cite{Clean-label backdoor attacks on video recognition models} extended the clean label attack to video recognition models by adopting a universal adversarial trigger as the backdoor trigger pattern. Recently, many backdoor attacks have been researched in other tasks or paradigms. 

\lpz{In nlp tasks.} In transfer learning, Yao et al.~\cite{Latent Backdoor Attacks on Deep Neural Networks} proposed the latent attack to inject the incomplete backdoors into a Teacher model, and numerous student models will inherit the backdoors by transfer learning, as long as the downstream tasks of student models include the label targeted by the backdoor, the backdoor will be complete and activated. Some other attacks~\cite{XXXXXXX} are also proposed. In reinforcement learning, Yang et al.~\cite{Design of intentional backdoors in sequential models} proposed a backdoor attack to make models learn an adversarial policy which makes the models perform target sequential actions chosen by attackers besides the normal policy to perform by the benign models. Some other backdoor attacks~\cite{XXX} in reinforcement learning are also proposed. In the self-supervised learning, Jia et al.~\cite{badencoder} proposed BadEncoder to inject backdoor into a pre-trained image encoder, so the downstream classifiers trained based on the encoder for various downstream tasks will inherit the backdoor. Moreover, backdoor attacks in other tasks or paradigms have been also researched, including vision transformers, quantization, 3D point cloud, and so on.

In the Data-free scenarios, Liu et al.~\cite{liu2017trojaning} propose Trojaning Attack, which first generates a universal trigger by reversing the target DNN and retraining the DNN with the generated dataset containing poisoned instances stamped with the reversed trigger to inject backdoors. However, Trojaning attack needs to generate a dataset by reversing one image for each label and then fine-tune parameters, which is too costly on large models with many parameters and labels, such as \todo{XXXX}. Our backdoor attack consumes much fewer resources and can also embed backdoors in a data-free way. Recently, Lv et al.~\cite{DBIA} proposed DBIA to effectively backdoor the emerging vision transformer models by leveraging the inherent attention to generate triggers and injecting the backdoor using the poisoned surrogate dataset, however, DBIA can only apply to the models with the attention mechanism, not apply to the classic convolution neural networks. Our backdoor attack has better applicability against multiple model structures compared with DBIA.

\subsection{Backdoor Defenses in DNNs}
\label{subsec:backdoor-defenses}

Based on a general assumption that the neurons activated by benign and trigger inputs are different or separable, Liu et al.~\cite{fine-pruning} proposed to remove potential backdoor by firstly pruning the chosen the DNNs' neurons that contribute least to the main task (i.e., contribute most to backdoor task). After pruning, fine-tuning is used to restore model performance and further removing backdoor. Nonetheless, this method substantially degrades the model accuracy [XXX] owning to many pruned neurons are not only activated by trigger inputs but also activated by benign inputs. 
To reinforce models, Du et al. [XXX] proposed to apply differential privacy when performing model training to facilitate the detection of outliers, because poisoned data can be viewed as outliers.

Neural Cleanse~\cite{wang2019neural} examines whether a DNN model is backdoored by reversing the potential trigger patterns towards each label and identifying the backdoor trigger and its label based on outlier detection (i.e., a substantially smaller trigger to cause misclassifications). Then it fine-tunes backdoored DNNs with the clean samples and the backdoor samples stamped with reversed trigger to obtain benign DNNs, like adversarial training. trigger. Then, TABOR extended Neural Cleanse by utilizing various regularization when solving optimizations. However, Neural Cleanse and Tabor may consume too much resource for the models with numerous parameters and labels. 

ABS~\cite{Liu2019ABSSN} proposed to scan a DNN to determine whether it is backdoor by analyzing the compromised neurons contributing to the backdoors based on the assumption that the neurons that substantially elevate the activation of a particular output label regardless of the provided inputs, and generate the reversed trigger using the stimulation analysis to confirm the neurons compromised. However, it may not be suitable for large models with numerous neurons due to the training cost. 

Colouri et al. [XXX] judged whether the model is clean or backdoor by query a small set of specifically chosen image inputs named as universal litmus patterns (ULPs), then the logits (from the penultimate layer) are concatenated as feature input to the meta-classier, which will give a predict about whether the model is compromised. 

Xu et al. [XXX] proposed to use meta-classifier to predict whether a new model is clean or not. Firstly, it generate a set of benign and Trojaned shadow models as the training dataset of meta-classifier. Particularly, the shadow trojaned models are trained over diverse trojan attack settings (such as trigger patterns and backdoor goals) to approximate the general distribution of trojaned models. Moreover, many query inputs are made to each shadow model by back propagation, and the outputs of the shadow model are concatenated as the inputs of the meta-classifier model, the meta-classifier model will give a binary result to whether a model is clean or not. 

Moreover, both SentiNet~\cite{chou2018sentinet} and Februus~\cite{doan2020februus} discover the trigger by utilizing Grad-GAM~\cite{selvaraju2017grad} to locate contiguous regions of an input image that contribute significantly to the classification label.

%Moreover, both SentiNet~\cite{chou2018sentinet} and Februus~\cite{doan2020februus} utilize Grad-GAM~\cite{selvaraju2017grad} to discover the contiguous regions of an input image that contribute significantly to the classification result and conclude that such regions are highly likely to contain a trigger. 

==> sections/Related_work.tex <==
\section{Related Work}
\label{sec:Related work}
%-------------------------------------------------------------------------------
%\shengzhi{Do a thorough literature review for related works, especially those about watermarking neural networks. Make sure you will not miss important related works.}
\vspace{2pt}\noindent\textbf{Watermarking neural networks.} 
%With the development of artificial intelligence technology and the improvement of computing power, DNN is now widely used in various fields. The model of DNN is an invaluable IP for its owners because DNN training requires both advanced algorithms and high-quality data sets, as well as significant computational costs. 
Uchida et al.~\cite{uchida2017embedding} proposed the idea of utilizing a parameter regularizer to embed a watermark in the parameter space of the model and retrieved it during ownership verification. However, such an approach is vulnerable to statistical analysisattack~\cite{wang2019attacks},  because the layer's parameter variance with embedded watermark is more significant than other layers without watermark. In contrast, our EPH was embedded into nearly every layer of DNN-watermarked and occupied only a small portion of its parameter space, so the variances between the layers with and without EPH are not entirely different, thus ensuring stealthiness. 

%\shengzhi{what are ghost signature and tampering attacks?} 
%\shengzhi{If you mention their approach suffer from ghost signature and tampering attacks, you need to say how our approach defeat those two attacks.}
%introduced the idea of digital of watermark, and first proposed a framework for embedding the watermark in model parameters, which is applicable to the protection of white box models. These work provide a research direction for the protection of the IP of DNN, and the latter related research all revolves around how to embed a watermark on the model. However, the premise of white box watermarking is to have access to all parameters of the target model, and DNNs are usually deployed for remote access, so the assumption is difficult to guarantee in reality.  

Recently, backdoor-based watermarking approaches have been proposed to probe black-box or grey-box neural network models that are suspects of IP infringement~\cite{adi2018turning}, \cite{zhang2018protecting}, \cite{guo2018watermarking}, \cite{rouhani2018deepsigns}. Adi et al.~\cite{adi2018turning} embedded a set of abstract images with predefined labels into DNN models to build the trigger set, which acted as digital watermarks (only known to model owners) against the suspect models. Zhang et al.~\cite{zhang2018protecting} enriched the training dataset by adding content, noise, or irrelevant class examples as triggers, and leveraged them as model watermarks. Guo et al.~\cite{guo2018watermarking} proposed a watermarking approach similar to~\cite{zhang2018protecting} that can be used on embedded devices.
%Zhang et al.~\cite{zhang2018protecting} generalized digital watermarking as a method to hide secret information in digital media to protect the ownership of those media data, and proposed a watermarking approach for model ownership verification based on image recognition, which generates a sample trigger set of backdoor watermarks by adding content, noise, or irrelevant class examples to the raw training data. 
%Rouhani et al.~\cite{rouhani2018deepsigns} watermarked both white-box and black-box models by selecting pairs of random images and random labels as watermarks (key samples) and embedding them in the probability density function of the activation set of the target layer. \shengzhi{How can this be black-box?} 
However, the backdoor watermark approaches proposed above are non-blind watermark, which either fails to defend against evasion attacks~\cite{hitaj2018have} or does not explicitly address the problem of fraudulent ownership claim. Evasion attack~\cite{hitaj2018have} evades backdoor-based watermark verification by training a powerful detector to identify key samples in the trigger set of owners, and returning a random label rather than the predefined label when it detects a key sample used as input. 

To overcome the ``non-blind'' problem, backdoor-based blind watermarking approach \cite{namba2019robust}, \cite{li2019prove} has been proposed. Namba et al.~\cite{namba2019robust} utilized the original samples in the training dataset as watermarks by changing their labels. Li et al.~\cite{li2019prove} built watermarks by integrating a specific logo into the original samples and changing their labels. Merrer et al.~\cite{le2019adversarial} proposed a zero-bit watermarking algorithm based on adversarial examples. It fine-tunes the DNN-to-be-protected, so that the produced DNN model contains certain true/false adversarial examples, which can be used as secret keys to achieving ownership verification of the DNN models. These approaches still cannot deal with the fraudulent claims of ownership, since attackers can still pretend to be owners by utilizing adversarial samples to build their own trigger set. Different from these studies, our HufuNet can achieve high robustness and security.

%\todo{Such watermarking approach is based on adversarial training, which is initially as a defense against adversarial examples and also commonly used to improve the generalization performance of neural networks~\cite{miyato2018virtual}. For this reason, this watermarking method can falsely determine models without watermark as models with a watermark~\cite{namba2019robust}}. \lpz{Those works also have a vulnerability that each model essentially has infinite such keys, therefore everyone can claim the ownership of the DNN models with any K, that is fraudulent claims of ownership. In contrast, our HufuNet can resist fraudulent claims of ownership, such as forging a HufuNet.}

\vspace{2pt}\noindent\textbf{Counterattacks against watermarking.} Uchida et al. \cite{uchida2017embedding} proposed to fine-tune or prune the DNN model to modify its parameters, thus removing the embedded watermark.
%Because of the increasing robustness of existing watermarking techniques, watermarks can be successfully validated even when the DNN model itself fails due to pruning and fine-tuning.
Wang et al.~\cite{wang2019attacks} proposed to reveal any watermark based on the change of statistical distribution of parameters of the layer where the watermark is embedded. Yang et al.~\cite{yang2019effectiveness} demonstrated that distillation-based attacks can be effective to perform watermark elimination, based on the premise that the adversaries have plenty of data to fine-tune the model. Chen et al.~\cite{chen2019leveraging} proved that the well-designed fine-tuning method can remove the watermark without compromising the function of the model with a large learning rate and unlabeled data. Hitaj et al.~\cite{hitaj2018have} proposed a method of evasion attacks against backdoor watermarks, which evade the homeowner's verification, thereby avoiding the discovery of model theft.
%Further, Chen et al.~\cite{chen2019refit} proposed a framework that removes the watermark based on fine-tuning, named REFIT, with limited data.
Although these counterattacks significantly threaten the backdoor-based watermarking, our design has better robustness against them. 

%\vspace{5pt}\noindent\textbf{Model stealing.} \shengzhi{Consider deleting the below related works, due to: 1. not quite relevant to watermarking, 2. space limitation.} Model stealing attack learns parameters~\cite{tramer2016stealing}, hyperparameters~\cite{wang2018stealing}, or architectural information~\cite{oh2019towards} of the target model, thus constructing a model with similar performance. Tramer et al.~\cite{tramer2016stealing} proposed a models stealing attack via API prediction, using non-adaptive, random queries to infer the parameters of the  target model. Orekondy et al.~\cite{Orekondy_2019_CVPR} proposed a functionality stealing attack to extract DNN attributes based on the input and output pairs of the target model，which are used to train a ``knockoff'' model. Jagielski et al.~\cite{jagielski2020high} proposed a functionally-equivalent model extraction attack by improving the learning-based attack's query efficiency. Their prediction matches the target model on all test samples without training their model weights. Model inversion~\cite{fredrikson2014privacy,fredrikson2015model,papernot2016towards,melis2019exploiting} relies on the output of some hidden input to infer certain features of it. Fredrikson et al.~\cite{fredrikson2015model} proposed a model reversal attack, which enables the recovery of images from the training dataset of the target DNN models. Melis et al.~\cite{melis2019exploiting} showed that in collaborative learning scenarios, attackers can infer sensitive attributes, e.g., gender, related to the new training dataset after the target model is updated with such dataset. Shokri et al.~\cite{shokri2017membership} first introduced membership inference attack, which aims to determine whether a given data sample is included in the training data. Salem et al.~\cite{salem2018ml} extended \cite{shokri2017membership} by relaxing its requirements, thus a more generic approach. Shokri et al. generated training data for the target model by using a shadow model to simulate the behavior of the target model. Yeom et al.~\cite{yeom2018privacy} demonstrated that under the premise that attackers can access the target model and know the average training loss of the model, overfitting may directly lead to membership inference attack.

==> sections/Stealthiness.tex <==
\section{Evading Adaptive Attackers}


\subsection{Knowledge of our watermark}



\noindent\textbf{Proposed Defenses}

\subsection{Neural Cleanse}


\subsection{ABS}


\subsection{Anomaly Detection}

==> template/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

